Assessing LLM Reasoning Steps via Principal Knowledge Grounding

Step-by-step reasoning has become a standard approach for large language models (LLMs) to tackle complex tasks. While this paradigm has proven effective, it raises a fundamental question: How can we verify that an LLM's reasoning is accurately grounded in knowledge? To address this question, we introduce a novel evaluation suite that systematically assesses the knowledge grounding of intermediate reasoning. Our framework comprises three key components. (1) Principal Knowledge Collection, a large-scale repository of atomic knowledge essential for reasoning. Based on the collection, we propose (2) knowledge-grounded evaluation metrics designed to measure how well models recall and apply prerequisite knowledge in reasoning. These metrics are computed by our (3) evaluator LLM, a lightweight model optimized for cost-effective and reliable metric computation. Our evaluation suite demonstrates remarkable effectiveness in identifying missing or misapplied knowledge elements, providing crucial insights for uncovering fundamental reasoning deficiencies in LLMs. Beyond evaluation, we demonstrate how these metrics can be integrated into preference optimization, showcasing further applications of knowledge-grounded evaluation.

==> tables/correlation.tex <==
\begin{table}[]
\centering
\small
\begin{tabular}{lcccc}
\toprule
 & KA & WKA & KR & WKR \\ \midrule
Correlation & 0.5069 & 0.5077 & 0.1813 & 0.2115 \\ \bottomrule
\end{tabular}%
\caption{Correlation between answer and KA, WKA, KR, WKR}
\end{table}

